Flavor Anisotropy in the High-Energy Astrophysical Neutrino Sky

High-energy astrophysical neutrinos, with TeV--PeV energies, offer unique insight into astrophysics and particle physics. Their incoming directions and flavor composition -- i.e., the proportion of electron, muon, and tau neutrinos in their flux -- are, individually, rewarding observables. Combined, they offer new opportunities, hitherto unexplored, that we expose for the first time. Anisotropy in the arrival directions of electron, muon, and tau neutrinos may reveal multiple populations of neutrino sources, differently distributed in the sky, and test whether neutrinos of different flavor propagate preferentially along certain directions, such as expected from breaking Lorentz invariance. Using 7.5 years of public IceCube High-Energy Starting Events, we make the first measurement of the directional flavor composition of high-energy astrophysical neutrinos, constrain the presence of flavor dipoles and quadrupoles, and improve constraints on "compass asymmetries" introduced by Lorentz invariance violation. In the near future, upcoming neutrino telescopes will improve these measurements across the board.

==> spare.tex <==
%\subsection{Sources of anisotropy}\label{sec:aniso_cources}
Beyond the Standard Model physics (BSM) allows for the possibility of a wide range of neutrino phoenomenology. Models considering the possibility of Lorentz invarience violation \cite{}, or neutrino interactions with galactic dark matter \cite{} predict possible anisotropy in neutrino flavor ratios \cite{}. However, current attempts to constrain such behaviors considered mostly all-flavor anisotropies \cite{}. Exploring the flavor structure opens a new window to constrain the parameter spaces of these models. Phoenomenologically, the flavor flux at Earth is derived by propagating the source flux over a redshift range and accounting for flavor oscillations along the way \cite{}. We model the flavor $\alpha$ flux at Earth as given in \cite{}:
\begin{equation}
    \begin{split}
        \frac{\partial\Phi_\alpha}{\partial E} &= \int \,dz\,\frac{dV}{dz}\, n\, J\,\sum f_{s,\beta}\,P_{\alpha\beta}.\\
    \end{split}
\end{equation}


...



\begin{equation}
\begin{split}
    \mathcal{D}^{\alpha\,\beta} &= \frac{\Phi_\alpha-\left\langle \Phi_\alpha \right\rangle}{\left\langle \Phi_\alpha \right\rangle} - \frac{\Phi_\beta-\left\langle \Phi_\beta \right\rangle}{\left\langle \Phi_\beta \right\rangle}\\
                                &= \sum_{\ell>0,m} d^{\alpha\,\beta}_{\ell\,m}\, Y_{\ell\,m},
\end{split}
\end{equation}
where $d^{\alpha\,\beta}_{\ell\,m} = a^\alpha_{\ell\, m}-b^\beta_{\ell\,m}$. As this quantity is invariant to any source distribution for $\ell>0$, it is a direct measure of any anisotropy in neutrino oscillation behavior, as well as anisotropies in the flavor ratios at the sources. We will therefore also report its detection prospects, measured with the flavor difference power spectrum, $C^{\alpha\,\beta}_{\ell}$, defined equivalently to Equation (\ref{eq:pow_sp}).





\section{Flavor anisotropy}
\label{sec:aniso_model}

\subsection{Flavor sky harmonic expansion}
We consider the all-flavor neutrino flux to be isotropic at Earth. The flavor flux at Earth for each flavor $\alpha$ was decomposed as:
\begin{equation}\label{eq:flav_flux_earth}
    \Phi_\alpha = \frac{\Phi_0}{4\pi}f_\alpha\left[1+\sum_{\ell>0,m} a^\alpha_{\ell \, m} Y_{\ell\, m}\right]\left(\frac{E}{1\,\text{GeV}}\right)^{-\gamma},
\end{equation}
where $Y_{\ell\, m}$ denote the real-valued spherial harmonic functions; $a^\alpha_{\ell \, m}$ is the $\ell,m$ anisotropy harmonic moment; $f_\alpha$ is the mean flavor ratio for flavor $\alpha$; and $\Phi_0$ is the all-sky, all-flavour flux normalisation. The all-sky flavor ratios obey the identity $\sum_\alpha f_\alpha = 1$. Since we assume the all-flavor flux is isotropic, this imposes the further condition that, for all $\ell,m$:
\begin{equation}\label{eq:tot_iso_cond}
    \sum_\alpha f_\alpha\, a^\alpha_{\ell,m} = 0.
\end{equation}

In this decomposition, $a^\alpha_{\ell\, m}$ describe the directional anisotropy of the flavor ratio away from its mean all-sky value. Isotropy for flavor $\alpha$ is recovered when $a^\alpha_{\ell\,m} = 0\,\forall \, \ell>0,m$. The measure that we adopt to report total anisotropy is the harmonic power spectrum measure:
\begin{equation}\label{eq:pow_sp}
    C^\alpha_\ell = \frac{1}{2\ell+1}\sum_{m=-\ell}^\ell \left|a^\alpha_{\ell\,m}\right|^2.
\end{equation}

We call $C^\alpha_\ell$ the $\ell$-pole power of anisotropy. Trivially, isotropy for flavor $\alpha$ is recovered when $C^\alpha=0\,\forall\,\ell>0$. In this prescription, anisotropies captured by $a_{\ell\,m}$ couple total neutrino anisotropies (combining all flavors), and the anisotropies of the flavor ratios. However, the difference in the anisotropy terms of different flavors factors out the all-flavor anisotropies, and the resulting function is everywhere-zero, unless anisotropies in the flavor ratios are non-zero for any of the poles $\ell>0$. We therefore define a quantity, the $\alpha,\beta$-difference, which captures the difference in the anisotropy terms:

\begin{equation}
\begin{split}
    \mathcal{D}^{\alpha\,\beta} &= \frac{\Phi_\alpha-\left\langle \Phi_\alpha \right\rangle}{\left\langle \Phi_\alpha \right\rangle} - \frac{\Phi_\beta-\left\langle \Phi_\beta \right\rangle}{\left\langle \Phi_\beta \right\rangle}\\
                                &= \sum_{\ell>0,m} d^{\alpha\,\beta}_{\ell\,m}\, Y_{\ell\,m},
\end{split}
\end{equation}
where $d^{\alpha\,\beta}_{\ell\,m} = a^\alpha_{\ell\, m}-a^\beta_{\ell\,m}$. This difference is a direct probe into the angular structure of the flavor ratios, allowing us to directly constrain processes which generate flavor ratio anisotropies. 











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Ice Cube is the largest operating neutrino telescope to date, capable of distinguishing three different event morphologies, correlated to each neutrino flavor (cascades, tracks and double cascades) \cite{}. Ice Cube is a Cherenkov detector; it uses photomultipliers to capture the radiative light of the products of deep inelastic scatter neutrino--nucleon interactions in the ice. For this reason, it is generally unable to differentiate between neutrino and antineutrino events. The final state particles of these interactions are charged leptons and hadrons, which emit Cherenkov radiation as they propagate through the ice. From the amount of light collected, and its geometric and temporal distribution, Ice Cube infers the incoming neutrino energy and arrival direction. The energy distribution in the ice can is categorised into the three event morphologies. Cascades are roughly spherical, highly localised events, mostly produced by charged-current (CC) interactions. They produce an outgoing charged lepton, and in the case of a $\nu_e$ interaction, this electron initiates an electromagnetic shower that is highly localised. In these events, nearly all the energy of the final state particles is deposited in the detector, leading to good energy resolution, however, the mostly-spherical geometry of the event leads to poorer angular resolution. When the initial neutrino interacts as a $\nu_mu$, the resulting muon traverses the detector while stochastically depositing energy, which is observed as a long track in the detector. Hence, track events are strongly correlated to $\nu_\mu$ events. Double cascades occur when two cascade events can be temporally correlated, and are mostly produced when a neutrino interacts as a $\nu_\tau$, producing a charged $\tau$ lepton in the first cascade, which traverses some length before decaying and leaving a second cascade-like morphology. Both tracks and double cascades have an asymmetric structure compared to cascades, producing comparatively better angular resolution. Overall, the three morphologies have cross-feed from all three flavour interactions, so the flavour composition of the detected neutrinos can only be statistically inferred \cite{}. 

Ice Cube has discovered a flux of high-energy astrophysical neutrinos \cite{}, and has subsequently released an associated public data sample and Monte Carlo (MC). This High Energy Starting Event (HESE) sample was collected over a timespan of 7.5 years and is comprised of 102 events with energies $>10^4$ GeV \cite{}. The event arrival distributions are attenuated by the Earth, but events from the northern hemisphere are still observable, allowing us to make a full-sky analysis. A classification of event morphologies and their flavor compositions in the MC is given in Figure \ref{fig:morphologies}. Due to the low number of double cascades, correlating to $\nu_\tau$ events and the relatively high cross-feed from $\nu_\tau$ to cascades, there is substantial correlation between $\nu_\tau$ and $\nu_e$ events.\\

The HESE MC consists of 821\,764 events simulated with an isotropic flux under the assumption of a $(1/3,1/3,1/3)$ flavour ratio at Earth. Their positional and energy resolutions are described in \cite{} and we discuss the effects of angular resolution on angular flux reconstruction in Appendix \ref{app:stat_valid}. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Many planned Ice Cube-like detectors are currently in various stages of deployment. Their addition to the global network of neutrino telescopes is an exciting prospect not only due to the improvement in the number of high-energy events observable, but also due to the distribution of detectors around the Earth, which helps compensate for the signal attenuation of each individual detector. Both factors can substantially enhance our sensitivity to the directional flavor composition. However, no public releases exist to date of the detection capabilities or efficiencies of these upcoming telescopes, so we chose to model their responses using the Ice Cube Monte Carlo, scaled to their effective area as a fraction of Ice Cube's effective area. We only consider the final projected effective area and data that is collected in 5-year increments. We copied the Ice Cube Monte Carlo modified to include azimuthal information (both true and reconstructed direction) for each considered detector (see Appendix \ref{sec:valid_mc_mod}). Then, for each detector's new Monte Carlo set, we shifted all events by the detector's latitude and longitude, so that the MC would reflect the attenuation as seen by that detector. We then made detector-specific modifications in two cases. For KM3NET, we adjusted the angular uncertainty on the reconstructed arrival direction by shifting the reconstructed direction closer to the true event direction by a factor of $1/3$ for cascades, to reflect the $\approx 10^\circ$ angular resolution for cascades in water, as opposed to $\approx 30^\circ$ in ice. For TAMBO, we removed all MC events except double cascades produced by $\nu_\tau$ events, due to its specific design. The considered detectors, their effective areas and projected data release dates are shown in Figure \ref{fig:future-detectors}. Section \ref{sec:future_detector_descriptions} describes the considered detectors in more detail.



%%%%%%%%%%%%%%%%%%%
\begin{figure}
    \centering
    \includegraphics[width = 0.45\textwidth]{figures/allflav_iso_disco_fin.pdf}
    \caption{\justifying The flavor-dependent dipole (solid line) and quadropole (dashed line) polar ($m=0$) harmonic moment discoverable at a 90\% C.L. Points recovered with all detectors, whose Ice Cube-equivalent exposure is given on the top axis. The 2040 points indicated with left- and right-facing triangles represent the values discoverable with only the Ice Cube detector at 2040. The left axis shows the sky maximum as a percentage of the mean sky value, when only the polar dipole has the values given on the left axis.}
    \label{fig:sig2_disco}
\end{figure}

\begin{figure}
    \includegraphics[width = 0.45\textwidth]{figures/allflav_iso_constraints_fin.pdf}
    \caption{\justifying The flavor-dependent dipole (solid line) and quadropole (dashed line) power consistent with isotropy at a 90\% confidence level (C.L.), recovered assuming truly isotropic flavor composition at Earth. Points recovered with all detectors, whose Ice Cube-equivalent exposure is given on the top axis. The 2040 points indicated with left- and right-facing triangles represent the values constrainable with only the Ice Cube detector at 2040. The left axis shows the average value of the sky maximum as a percentage of the mean sky value, when only the dipole power has the values given on the left axis.}
    \label{fig:iso_constraints}
\end{figure}





\section{LIV flux at Earth}

The equation accounting for the propagation of each neutrino flavor to Earth is given as in \cite[Eq.B4]{Bustamante:2016ciw}:

\begin{equation}
    \begin{split}
        \Phi_\alpha &= \int \,dz\frac{dV}{dz}\, n_\alpha(E(1+z)) J(E(1+z))\sum f_{s,\beta}P_{\alpha\beta}(E(1+z))\\
        &= \frac{\Phi_0}{E^2}\int \,dz\, \frac{\rho_{src}(z)}{h(z)(1+z)^2}[E(1+z)]^{2-\gamma}\sum f_{s,\beta}P_{\alpha\beta}(E(1+z)),
    \end{split}
\end{equation}
where 
\begin{equation}
    \rho_{src}(z) = \left[(1+z)^{a\eta}+\left(\frac{1+z}{B}\right)^{b\eta} + \left(\frac{1+z}{C}\right)^{c\eta}\right]^{1/\eta}
\end{equation}
and
\begin{equation}
    h(z) = H_0\sqrt{\Omega_m(1+z)^3+\Omega_\Lambda}
\end{equation}
and the $\rho$ parameters are set as in \cite[Eq.5]{Yuksel:2008cu}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Posterior of $h_{lm}$ LIV coefficients}

The posterior of the vector of LIV coefficients $\boldsymbol{h} \equiv (h_{1,-1}, h_{1,0}, h_{1,1}, \dots, h_{l_{\rm max}, l_{\rm max}})$ is
\begin{equation}
\begin{split}
 \mathcal{P}({h})
 &=
 \int d\boldsymbol{a}~
 {\rm det}[\boldsymbol{J}(\boldsymbol{a})]~
 \delta[h-h(\boldsymbol{a})]~
 \pi(\boldsymbol{a}) \;,\\
 &= \int d\boldsymbol{a}~
 {\rm det}[\boldsymbol{J}(\boldsymbol{a})]~
 \boldsymbol{\delta}[\boldsymbol{a}_h-\boldsymbol{a}]~
 \pi(\boldsymbol{a})\\
 &= {\rm det}[\boldsymbol{J}(\boldsymbol{a}_h)]
 \pi(\boldsymbol{a}_h),
 \end{split}
\end{equation}
(where $\boldsymbol{a}_h \ | \ h(\boldsymbol{a}_h) = h$)\\
where $\boldsymbol{a} \equiv (a_{1,-1}, a_{1,0}, a_{1,2}, \ldots, a_{l_{\rm max}, l_{\rm max}})$ are the coefficients of the spherical-harmonics expansion of the sky, $\boldsymbol{h}(\boldsymbol{a})$ is the value of the list of LIV coefficients inferred from the sky anisotropy when the values of the spherical-harmonics coefficients are $\boldsymbol{a}$, $\pi(\boldsymbol{a})$ is the prior on $\boldsymbol{a}$, and $\boldsymbol{J} \equiv \left( \partial \boldsymbol{h} / \partial \boldsymbol{a} \right)$ is the Jacobian. \BT{this doesn't work; see derivation following first line. We do not use the $\boldsymbol{a}$ posteriors in this derivation. Also, $h(\boldsymbol{a})$ is not a function we can analytically or numerically evaluate since $\boldsymbol{a}(h)$ is the correspondence that we have, and it is not invertible as it is not surjective.}\\


To constrain LIV anisotropy-generating parameters, we considered each matrix dimension, as well as LIV harmonic matrix and its entries independently. Each scalar $h_{\ell m}^{\alpha\beta}$ generates an line element $\boldsymbol{a}$ in the space of harmonic moments of the anisotropy differences on the sky. These sky moments can be directly compared to those whose posteriors we have recovered with our fits. The posterior sky harmonics can be seen as a subset $\Psi \subset  \mathbb{R}^{\ell_{max}^2+2\ell_{max}}$, parameterised by $\tau$ which we choose such that $\boldsymbol{a}(\tau) = \boldsymbol{a}(h)\, \forall \, h\in \mathbb{R}$. We recover the posterior of $h_{\ell m}^{\alpha\beta} = h$ by:
\begin{equation}
    \begin{split}
        \mathcal{P}({h}) &= \int_{\Psi} d\boldsymbol{a}\ 
                            \mathcal{L}(h|\boldsymbol{a}) \mathcal{P}(\boldsymbol{a})\\
                         &= \int_{-\infty}^{\infty} d\tau\ 
                            \mathcal{L}(h|\boldsymbol{a}(\tau)) \mathcal{P}(\boldsymbol{a}(\tau))\, ||D_\tau {\boldsymbol{a}}||\\
                         &= \int_{-\infty}^{\infty} d\tau\ 
                            \mathcal{L}(h|\boldsymbol{a}(\tau)) \mathcal{P}(\boldsymbol{a}(\tau))\, ||D_\tau {\boldsymbol{a}}||\\
                         &= \int_{-\infty}^{\infty} d\tau\ 
                            \delta(\tau-h) \mathcal{P}(\boldsymbol{a}(\tau) )\, ||D_\tau {\boldsymbol{a}}||\\
                         &= \mathcal{P}(\boldsymbol{a}(h))\,||D_\tau {\boldsymbol{a}}||(h)
    \end{split}
\end{equation}
where $\mathcal{P}(\boldsymbol{a})$ is the posterior of the sky harmonics, and $||D_\tau {\boldsymbol{a}}||(h)$ is the norm of the derivative of the pullback of $\boldsymbol{a}$ wrt $\tau$, evaluated at $h$.
